SIGNED: A Challenge-Response Based Interrogation Scheme for Simultaneous Watermarking and Trojan Detection

The emergence of distributed manufacturing ecosystems for electronic hardware involving untrusted parties has given rise to diverse trust issues. In particular, IP piracy, overproduction, and hardware Trojan attacks pose significant threats to digital design manufacturers. Watermarking has been one of the solutions employed by the semiconductor industry to overcome many of the trust issues. However, current watermarking techniques have low coverage, incur hardware overheads, and are vulnerable to removal or tampering attacks. Additionally, these watermarks cannot detect Trojan implantation attacks where an adversary alters a design for malicious purposes. We address these issues in our framework called SIGNED: Secure Lightweight Watermarking Scheme for Digital Designs. SIGNED relies on a challenge-response protocol based interrogation scheme for generating the watermark. SIGNED identifies sensitive regions in the target netlist and samples them to form a compact signature that is representative of the functional and structural characteristics of a design. We show that this signature can be used to simultaneously verify, in a robust manner, the provenance of a design, as well as any malicious alterations to it at any stage during design process. We evaluate SIGNED on the ISCAS85 and ITC benchmark circuits and obtain a detection accuracy of 87.61\% even for modifications as low as 5-gates. We further demonstrate that SIGNED can benefit from integration with a logic locking solution, where it can achieve increased protection against removal/tempering attacks and incurs lower overhead through judicious reuse of the locking logic for watermark creation.

==> analysis.tex <==
\section{Security Analysis}
\label{sec:analysis}
In this section, we analyze the security of~\signed framework by proposing a hypothetical attack and discuss additional countermeasures for preventing the same. We have shown in section~\ref{sec:results} that our proposed framework detects cloning, and counterfeiting attacks. Additionally, we have also demonstrated in Figure~\ref{fig:davsfs} that~\signed can also detect malicious alterations to the circuit. However, an attacker at the foundry or the design house could maliciously try to remove the digest logic.

In order to nullify the attacker's advantage we hide the digest logic by employing logic-locking techniques. In our current framework, we employ combinational logic locking to hide the signature of the digest logic. This approach would not incur any significant overheads. Since the digest logic is not a part of the critical path, it would not incur any delay overheads. The digest logic would only be triggered during the authentication phase and thus would not be always activated, thereby reducing the power overheads. The locking technique would incur a slight area penalty due to the transformation of the digest logic. However, this transformation could be further optimized by employing sequential locking techniques. 






